StableKD: Breaking Inter-block Optimization Entanglement for Stable Knowledge Distillation

Knowledge distillation (KD) has been recognized as an effective tool to compress and accelerate models. However, current KD approaches generally suffer from an accuracy drop and/or an excruciatingly long distillation process. In this paper, we tackle the issue by first providing a new insight into a phenomenon that we call the Inter-Block Optimization Entanglement (IBOE), which makes the conventional end-to-end KD approaches unstable with noisy gradients. We then propose StableKD, a novel KD framework that breaks the IBOE and achieves more stable optimization. StableKD distinguishes itself through two operations: Decomposition and Recomposition, where the former divides a pair of teacher and student networks into several blocks for separate distillation, and the latter progressively merges them back, evolving towards end-to-end distillation. We conduct extensive experiments on CIFAR100, Imagewoof, and ImageNet datasets with various teacher-student pairs. Compared to other KD approaches, our simple yet effective StableKD greatly boosts the model accuracy by 1% ~ 18%, speeds up the convergence up to 10 times, and outperforms them with only 40% of the training data.

==> tabs/IN_300.tex <==
\begin{table}[t]
% \vspace{-0.1in}
\centering
\resizebox{.9\linewidth}{!}{%
\begin{tabular}{c|ccc}
\toprule
     Models&w/o KD&KD&StableKD-5/3\\\midrule
     Swin-T \& Swin-S & 80.37 & 81.15&\textbf{82.61}
    \\ \bottomrule
\end{tabular}
}
%\vspace{-0.1in}
\caption{ImageNet results with 300 epochs. 
}
%\vspace{-0.1in}
    \label{tab:in_300}
\end{table}
